Binarized Knowledge Graph Embeddings

Tensor factorization has become an increasingly popular approach to knowledge graph completion(KGC), which is the task of automatically predicting missing facts in a knowledge graph. However, even with a simple model like CANDECOMP/PARAFAC(CP) tensor decomposition, KGC on existing knowledge graphs is impractical in resource-limited environments, as a large amount of memory is required to store parameters represented as 32-bit or 64-bit floating point numbers. This limitation is expected to become more stringent as existing knowledge graphs, which are already huge, keep steadily growing in scale. To reduce the memory requirement, we present a method for binarizing the parameters of the CP tensor decomposition by introducing a quantization function to the optimization problem. This method replaces floating point-valued parameters with binary ones after training, which drastically reduces the model size at run time. We investigate the trade-off between the quality and size of tensor factorization models for several KGC benchmark datasets. In our experiments, the proposed method successfully reduced the model size by more than an order of magnitude while maintaining the task performance. Moreover, a fast score computation technique can be developed with bitwise operations.

==> 2 <==
\subsection{Datasets and Evaluation Protocol}
\input{tables/dataset}
\input{tables/results_old}
\input{tables/results_new}
\input{figures/loss-acc}
\input{tables/results_comp}
\input{figures/time}
We evaluated the performance of our proposal in the standard
knowledge graph completion (KGC) task.
We used four standard datasets,
WN18, FB15k~\cite{transe}, WN18RR, and FB15k-237~\cite{conve}.
Table~\ref{tab:dataset} shows the data statistics\footnote{
Following \cite{simple,cano},
  %% improve the KGC performance of CP models,
for each triple $(e_i,e_j,r_k)$ observed in the training set,
we added its inverse triple $(e_j,e_i,r_k^{-1})$
also in the training set.}.

We followed the standard evaluation procedure
to evaluate the KGC performance:
Given a test triple $(e_i,e_j,r_k)$, we
corrupted it by replacing $e_i$ or $e_j$
with every entity $e_\ell$ in $\mathcal{E}$
and calculated $\theta_{i,\ell,k}$ or $\theta_{\ell,j,k}$.
We then ranked all these triples by
their scores in decreasing order.
To measure the quality of the ranking,
we used the mean reciprocal rank (MRR) and Hits at $N$~(Hits@$N$).
%We here reported results
%in both the filtered and raw settings~\cite{transe}
%for MRR, but only filtered values for Hits@$N$.
We here report only results in the filtered setting~\cite{transe},
which provides a more reliable performance metric in the presence of multiple correct triples.

\subsection{Experiment Setup}
\label{sec:expcond}
To train CP models, we selected the hyperparameters via
grid search such that the filtered MRR is maximized on the validation set.
For standard CP model,
we tried all combinations of $\lambda_A,\lambda_B,\lambda_C\in\{0.0001, 0\}$,
learning rate $\eta\in\{0.025, 0.05\}$,
and the embedding dimension $D\in\{15, 25, 50, 100, 150, \allowbreak 200, \allowbreak 300, \allowbreak 400, \allowbreak 500\}$ during grid search.
For our binarized CP model,
all combinations of $\lambda_A,\lambda_B,\lambda_C\in\{0.0001, 0\}$,
$\eta\in\{0.025, 0.05\}$, $\Delta\in\{0.3, 0.5\}$
and $D\in\{100,200,300,400,500\}$ were tried.
%\memo{The ensemble model isn't mentioned here at all. Its explanation must be placed here ore somewhere else, including how it aggregates the scores from 3 models.}
We randomly generated
the initial values of the representation vectors
from the uniform distribution
$U[-\frac{\sqrt{6}}{\sqrt{2D}},\frac{\sqrt{6}}{\sqrt{2D}}]$~\cite{init}.
The maximum number of training epochs was set to 1000.
For SGD training, negative samples were generated using
the local closed-world assumption~\cite{transe}.
The number of negative samples
generated per positive sample was 5 for WN18/WN18RR
and 10 for FB15k/FB15k-237.

%\memo{When we evaluated B-CP model, we also used {\it model ensemble}, which is the method
%using the sum of the scores in separately trained models.}
\textcolor{red}{When we evaluated B-CP model, we also used {\it model ensemble} which sums up
the scores in separately trained models.}


We implemented our CP decomposition 
systems in C++ and conducted all experiments on a 64-bit
16-Core AMD Ryzen Threadripper 1950x with 3.4GHz CPUs.
The program codes were compiled using GCC 7.3 with -O3 option.

\subsection{Results}
\subsubsection{Main Results}
We compared standard CP and binarized CP models~(B-CP)
with other state-of-the-art KGE models.
Table~\ref{tab:results_old} shows
the results on WN18 and FB15k,
and Table~\ref{tab:results_new} displays the results
on WN18RR and FB15k-237.
For most of the evaluation metrics,
our B-CP model~($D=400$) outperformed or was competitive
to the best baseline, although
with a small vector dimension ($D=200$),
B-CP showed tendency to degrade in its performance.
In the table, B-CP $(D=300\times 3)$ indicates
an ensemble of three different B-CP models (each with $D=300$).
This ensemble approach outperformed the baseline B-CP
constantly on all datasets.
Figure~\ref{fig:loss-acc} shows
training loss and accuracy versus epochs of training
for CP~($D=400$) and B-CP~($D=400$) on WN18RR.
The results indicate that CP is prone to overfitting with increased
epochs of training.
By contrast, B-CP appears less susceptible to
overfitting than CP.
%The results show that
%the quantization acts as regularizer.
%\memo{The data included in a knowledge graph is few compared with
%all possible triples, and therefore 
%the conventional CP decomposition method overfit to training data.}

\subsubsection{KGC Performance vs. Model Size}
We also investigated how our B-CP method
can maintain the KGC performance while reducing the model size.
For a fair evaluation, we also examined a naive vector quantization
method (VQ)~\cite{xnor} that can reduce the model size.
Given a real valued matrix ${\bm X}\in\Rset^{D_1\times D_2}$,
the VQ method solves the following optimization problem:
\begin{align*}
{\hat {\bm X}^{(b)}},{\hat \alpha}=\argmin_{{\bm X}^{(b)},\alpha}
{\|{\bm X}-\alpha{\bm X}^{(b)}\|_F^2}
\end{align*}
where ${\bm X}^{(b)}\in\{+1,-1\}^{D_1\times D_2}$ is a binary matrix
and $\alpha$ is a positive real value.
The optimal solutions ${\hat {\bm X}^{(b)}}$ and ${\hat \alpha}$
are given by $Q_1({\bm X})$ and $\frac{1}{D_1\times D_2} \| {\bm X} \|_{1}$,
respectively,
where $\|\cdot \|_1$ denotes $l_1$-norm,
and
$Q_1({\bm X})$ is a sign function whose behavior in each element $x$
of ${\bm X}$ is as per the sign function $Q_1(x)$.
%\begin{align*}
%\text{sign}(x)=\begin{cases}
%    1 & x\geq 0 \\
%    -1 & \text{otherwise}
%\end{cases}.
%\end{align*}
After obtaining factor matrices ${\bm A}$, ${\bm B}$ and ${\bm C}$
via standard CP decomposition,
we solved the above optimization problem independently for each matrix.
We call this method VQ-CP.

Table~\ref{tab:results_comp} shows the results
when the dimension size of the embeddings was varied.
While CP requires $64\times D$ and $32\times D$ bits per
entity and relation, respectively,
both B-CP and VQ-CP have only to take one thirty-second of them.
Obviously, the task performance dropped significantly
after vector quantization~(VQ-CP).
The performance of CP also degraded when reducing
the vector dimension from 200 to 15 or 50.
While simply reducing the number of dimensions degraded
the accuracy,
B-CP successfully reduced the
model size nearly 10- to 20-fold compared to CP and other KGE models
without performance degradation.
Even in the case of B-CP~$(D=300\times3)$, 
the model size was 6 times smaller than that of CP~$(D=200)$.

\subsubsection{Computation Time}
%While B-CP requires keeping the real-valued weights during training to do SGD updates,
%we can maintain just binary weights in testing time.
%The B-CP model contributes to not only model size reduction
As described in Section~\ref{sec:prop}, the B-CP model can
accelerate the computation of confidence scores by using the
bitwise operations~(XNOR and Bitcount).
%since
%the inner product between binary weight vectors
%can be efficiently implemented by the bitwise~(Xnor and Bitcount) operations.
To compare the score computation speed between CP~(Float) and
B-CP~(XNOR and Bitcount),
we calculated the confidence scores 100,000 times for both CP and B-CP,
varying the vector size $D$ from 10 to 1000 at 10 increments.
Figure~\ref{fig:time} clearly shows that
bitwise operations provide significant speed-up compared to
standard multiply-accumulate operations.
%The fast score computation would also bring great benefits
%to model training time.
%Actually, B-CP~$(D=500)$ was almost as fast as CP~$(D=200)$ over all
%datasets\footnote{
Since B-CP needs to keep and binarize real-valued vectors
during SGD updates, however,
it took about twice as long per training epoch as CP.
We suspect this is mainly because the GCC optimizer did not work well for
the quantization process.

\subsection{Evaluation on Large-scale Freebase}
\input{tables/ldataset}
To verify the effectiveness of B-CP over larger datasets,
we also conducted experiments on the Freebase-music
data\footnote{\url{https://datalab.snu.ac.kr/haten2/}}.
To reduce noises, we removed triples from the data
whose relation and entities occur less than 10 times.
The number of the remaining triples were 18,482,832
which consist of 138 relations and 3,025,684 entities.
We split them randomly into three subsets: 18,462,832
training, 10,000 validation, and 10,000 test triples.
We randomly generated 20,000 unknown triples and
added one half of them into validation
and the other into test triples as negative samples.
\memo{what do you mean by ``unknown'' triples? Here is a suggested rewrite, but I'm not sure if this is what is really meant: We randomly generated 20,000 triples that are not in the knowledge graph, and used them as negative samples; half of them were placed in the validation set, and the other half in the test set.}
\memo{But then, why no negative examples for training?}
Experiments were conducted under the same conditions we achieved
the best results on the small datasets.
We here report the triple classification accuracy.
\memo{sounds contradictory; if you use classification accuracy as the performance metric, the ``condition'' is not the same as the small datasets.}
Table~\ref{tab:ldata} gives the results.
As it was with the small datasets, 
the performance of CP~$(D=15)$ was again poor.
Meanwhile, B-CP successfully reduced the model size while achieving better
performance than CP~$(D=200)$.
These results show that B-CP is robust to the data size.
%B-CP also achieved better performance than CP on a large-scale dataset.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Local Variables:
%%% mode: latex
%%% TeX-PDF-mode: t
%%% TeX-engine: xetex
%%% TeX-master: "main"
%%% End:



==> figures/cp.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}[scale=0.75]
\pgfmathsetmacro{\cubex}{2}
\pgfmathsetmacro{\cubey}{2}
\pgfmathsetmacro{\cubez}{2}
\draw[black] (0,0,0) -- ++(-\cubex,0,0) -- ++(0,-\cubey,0) -- ++(\cubex,0,0) -- cycle;
\draw[black] (0,0,0) -- ++(0,0,-\cubez) -- ++(0,-\cubey,0) -- ++(0,0,\cubez) -- cycle;
\draw[black] (0,0,0) -- ++(-\cubex,0,0) -- ++(0,0,-\cubez) -- ++(\cubex,0,0) -- cycle;
\node (X) at (-1,-1.2,0) [above] {$\mathcal{X}$} ;
\node (subject) at (-1,-2,0) [below] {object} ;
\node (object) at (-2.2,-1,0) [rotate=90] {subject} ;
\node (relation) at (-1.85,0.5,0) [rotate=45] {relation} ;

%\pgfmathsetmacro{\cubex}{0.25}
%\pgfmathsetmacro{\cubey}{0.25}
%\pgfmathsetmacro{\cubez}{0.25}
%\draw[black] (-1,-1,-1) -- ++(-\cubex,0,0) -- ++(0,-\cubey,0) -- ++(\cubex,0,0) -- cycle;
%\draw[black] (-1,-1,-1) -- ++(0,0,-\cubez) -- ++(0,-\cubey,0) -- ++(0,0,\cubez) -- cycle;
%\draw[black] (-1,-1,-1) -- ++(-\cubex,0,0) -- ++(0,0,-\cubez) -- ++(\cubex,0,0) -- cycle;

\node (equal) at (1.2,-0.9,0) [above,font=\LARGE] {$=$} ;

\pgfmathsetmacro{\cubex}{0.3}
\pgfmathsetmacro{\cubey}{2}
\pgfmathsetmacro{\cubez}{2}
\draw[black] (2,0) -- ++(-\cubex,0) -- ++(0,-\cubey) -- ++(\cubex,0) -- cycle;
\draw[black] (2,0) -- ++(0,0) -- ++(0,-\cubey) -- ++(0,0) -- cycle;
\draw[black] (2,0) -- ++(-\cubex,0) -- ++(0,0) -- ++(\cubex,0) -- cycle;
\node (A) at (1.85,-2.4,0) [above] {$\bm{a}$} ;
\node (B) at (3.2,-0.3,0) [below] {$\bm{b}$} ;
\node (C) at (2.65,1.4,0) [below] {$\bm{c}$} ;

\pgfmathsetmacro{\cubex}{2}
\pgfmathsetmacro{\cubey}{0.3}
\pgfmathsetmacro{\cubez}{2}
\draw[black] (4.2,0) -- ++(-\cubex,0) -- ++(0,-\cubey) -- ++(\cubex,0) -- cycle;
\draw[black] (4.2,0) -- ++(0,0) -- ++(0,-\cubey) -- ++(0,0) -- cycle;
\draw[black] (4.2,0) -- ++(-\cubex,0) -- ++(0,0) -- ++(\cubex,0) -- cycle;

\pgfmathsetmacro{\cubex}{0.3}
\pgfmathsetmacro{\cubey}{2}
\pgfmathsetmacro{\cubez}{2}
\draw[black] (2,0.2,0) -- ++(-\cubex,0,0) -- ++(0,0,0) -- ++(\cubex,0,0) -- cycle;
\draw[black] (2,0.2,0) -- ++(0,0,-\cubez) -- ++(0,0,0) -- ++(0,0,\cubez) -- cycle;
\draw[black] (2,0.2,0) -- ++(-\cubex,0,0) -- ++(0,0,-\cubez) -- ++(\cubex,0,0) -- cycle;


\pgfmathsetmacro{\span}{3.5}
\pgfmathsetmacro{\cubex}{0.3}
\pgfmathsetmacro{\cubey}{2}
\pgfmathsetmacro{\cubez}{2}
\draw[black] (\span + 2,0) -- ++(-\cubex,0) -- ++(0,-\cubey) -- ++(\cubex,0) -- cycle;
\draw[black] (\span + 2,0) -- ++(0,0) -- ++(0,-\cubey) -- ++(0,0) -- cycle;
\draw[black] (\span + 2,0) -- ++(-\cubex,0) -- ++(0,0) -- ++(\cubex,0) -- cycle;
\node (A) at (\span + 1.85,-2.4,0) [above] {$\bm{a}$} ;
\node (B) at (\span + 3.2,-0.3,0) [below] {$\bm{b}$} ;
\node (C) at (\span + 2.65,1.4,0) [below] {$\bm{c}$} ;

\pgfmathsetmacro{\cubex}{2}
\pgfmathsetmacro{\cubey}{0.3}
\pgfmathsetmacro{\cubez}{2}
\draw[black] (\span + 4.2,0) -- ++(-\cubex,0) -- ++(0,-\cubey) -- ++(\cubex,0) -- cycle;
\draw[black] (\span + 4.2,0) -- ++(0,0) -- ++(0,-\cubey) -- ++(0,0) -- cycle;
\draw[black] (\span + 4.2,0) -- ++(-\cubex,0) -- ++(0,0) -- ++(\cubex,0) -- cycle;

\pgfmathsetmacro{\cubex}{0.3}
\pgfmathsetmacro{\cubey}{2}
\pgfmathsetmacro{\cubez}{2}
\draw[black] (\span + 2,0.2,0) -- ++(-\cubex,0,0) -- ++(0,0,0) -- ++(\cubex,0,0) -- cycle;
\draw[black] (\span + 2,0.2,0) -- ++(0,0,-\cubez) -- ++(0,0,0) -- ++(0,0,\cubez) -- cycle;
\draw[black] (\span + 2,0.2,0) -- ++(-\cubex,0,0) -- ++(0,0,-\cubez) -- ++(\cubex,0,0) -- cycle;

\node (plus) at (\span + 1.2,-0.9,0) [above,font=\LARGE] {$+$} ;

\pgfmathsetmacro{\span}{9}
\pgfmathsetmacro{\cubex}{0.3}
\pgfmathsetmacro{\cubey}{2}
\pgfmathsetmacro{\cubez}{2}
\draw[black] (\span + 2,0) -- ++(-\cubex,0) -- ++(0,-\cubey) -- ++(\cubex,0) -- cycle;
\draw[black] (\span + 2,0) -- ++(0,0) -- ++(0,-\cubey) -- ++(0,0) -- cycle;
\draw[black] (\span + 2,0) -- ++(-\cubex,0) -- ++(0,0) -- ++(\cubex,0) -- cycle;
\node (A) at (\span + 1.85,-2.4,0) [above] {$\bm{a}$} ;
\node (B) at (\span + 3.2,-0.3,0) [below] {$\bm{b}$} ;
\node (C) at (\span + 2.65,1.4,0) [below] {$\bm{c}$} ;

\pgfmathsetmacro{\cubex}{2}
\pgfmathsetmacro{\cubey}{0.3}
\pgfmathsetmacro{\cubez}{2}
\draw[black] (\span + 4.2,0) -- ++(-\cubex,0) -- ++(0,-\cubey) -- ++(\cubex,0) -- cycle;
\draw[black] (\span + 4.2,0) -- ++(0,0) -- ++(0,-\cubey) -- ++(0,0) -- cycle;
\draw[black] (\span + 4.2,0) -- ++(-\cubex,0) -- ++(0,0) -- ++(\cubex,0) -- cycle;

\pgfmathsetmacro{\cubex}{0.3}
\pgfmathsetmacro{\cubey}{2}
\pgfmathsetmacro{\cubez}{2}
\draw[black] (\span + 2,0.2,0) -- ++(-\cubex,0,0) -- ++(0,0,0) -- ++(\cubex,0,0) -- cycle;
\draw[black] (\span + 2,0.2,0) -- ++(0,0,-\cubez) -- ++(0,0,0) -- ++(0,0,\cubez) -- cycle;
\draw[black] (\span + 2,0.2,0) -- ++(-\cubex,0,0) -- ++(0,0,-\cubez) -- ++(\cubex,0,0) -- cycle;

\node (plus) at (\span -1,-0.9,0) [above,font=\LARGE] {$+$} ;
\node (plus) at (\span +1.2,-0.9,0) [above,font=\LARGE] {$+$} ;
\node (dot) at (\span +0.1,-0.9,0) [above,font=\LARGE] {$\cdots$} ;

\end{tikzpicture}
\caption{Illustration of a $D$-component CP model for
a third-order tensor $\bm{\mathcal{X}}$.}
\label{fig:cp}
\end{figure}

